SwiftTry: Fast and Consistent Video Virtual Try-On with Diffusion Models

Given an input video of a person and a new garment, the objective of this paper is to synthesize a new video where the person is wearing the specified garment while maintaining spatiotemporal consistency. Although significant advances have been made in image-based virtual try-on, extending these successes to video often leads to frame-to-frame inconsistencies. Some approaches have attempted to address this by increasing the overlap of frames across multiple video chunks, but this comes at a steep computational cost due to the repeated processing of the same frames, especially for long video sequences. To tackle these challenges, we reconceptualize video virtual try-on as a conditional video inpainting task, with garments serving as input conditions. Specifically, our approach enhances image diffusion models by incorporating temporal attention layers to improve temporal coherence. To reduce computational overhead, we propose ShiftCaching, a novel technique that maintains temporal consistency while minimizing redundant computations. Furthermore, we introduce the TikTokDress dataset, a new video try-on dataset featuring more complex backgrounds, challenging movements, and higher resolution compared to existing public datasets. Extensive experiments demonstrate that our approach outperforms current baselines, particularly in terms of video consistency and inference speed. The project page is available at https://swift-try.github.io/.

==> sections/checklist.tex <==
\newcommand{\answerYes}[1][]{\textcolor{black}{[Yes] #1}}
\newcommand{\answerNo}[1][]{\textcolor{black}{[No] #1}}
\newcommand{\answerPartial}[1][]{\textcolor{black}{[Partial] #1}}
\newcommand{\answerNA}[1][]{\textcolor{black}{[NA] #1}}

\section*{Reproducibility Checklist}
\begin{enumerate}

\item \textbf{This paper}:
    \item[] \textbf{Question:} Includes a conceptual outline and/or pseudocode description of AI methods introduced
    \item[] Answer: \answerYes 
    
    \item[] \textbf{Question:} Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper
    \item[] Answer: \answerYes

    
\item \textbf{Does this paper make theoretical contributions?} \answerNo

\item \textbf{Does this paper rely on one or more datasets?} \answerYes


    \item[] \textbf{Question:} A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
    \item[] Answer: \answerYes. We release a new dataset in this paper.
    
    \item[] \textbf{Question:} All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
    \item[] Answer:  \answerYes. We will publish after the paper acceptance.
    
    \item[] \textbf{Question:} All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (yes/no/NA)
    \item[] Answer:  \answerYes
    
    \item[] \textbf{Question:} All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (yes/partial/no/NA)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    \item[] Answer: \answerNA. All datasets used in this paper are publicly available.

\item \textbf{Does this paper include computational experiments?} \answerYes


    \item[] \textbf{Question:} Any code required for pre-processing data is included in the appendix. (yes/partial/no).
    \item[] Answer: \answerNo

    \item[] \textbf{Question:} All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
    \item[] Answer: \answerYes
     
    \item[] \textbf{Question:} All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
    \item[] Answer:  \answerYes
    
    \item[] \textbf{Question:} If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:} This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:}This paper states the number of algorithm runs used to compute each reported result. (yes/no)
    \item[] Answer: \answerYes
    
    \item[] \textbf{Question:}Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
    \item[] Answer: \answerNo
    
    \item[] \textbf{Question:} The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
    \item[] Answer: \answerNo
    
    \item[] \textbf{Question:} This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. (yes/partial/no/NA)
    \item[] Answer:  \answerYes
    
    \item[] \textbf{Question:} This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
    \item[] Answer: \answerYes
    
\end{enumerate}

